Ring Paxos: High-Throughput Atomic Broadcast

Atomic broadcast is an important communication primitive often used to implement state-machine replication. Despite the large number of atomic broadcast algorithms proposed in the literature, few papers have discussed how to turn these algorithms into efficient executable protocols. This paper focuses on a class of atomic broadcast algorithms based on Paxos, with its corresponding desirable properties: safety under asynchrony assumptions, liveness under weak synchrony assumptions, and resiliency-optimality. The paper presents two protocols, M-Ring Paxos and U-Ring Paxos, derived from Paxos. The protocols inherit the properties of Paxos and can be implemented very efficiently. We report a detailed performance analysis of M-Ring Paxos and U-Ring Paxos and compare them to other atomic broadcast protocols.

==> rpaxos.tex <==
%\begin{algorithmic}[1]
\line(1,0){240}
\begin{distribalgo}[1]
\small
\STATE \textbf{Algorithm 2: Ring Paxos} (for process $p$)
\vspace{1.5mm}
\STATE \emph{\underline{Phase~1 (coordinator)}}
\INDENT{\bc{Initialization}}
%\INDENT{\bc{\textbf{upon} receiving value $v$ from proposer}}
	\STATE \bc{increase \mv{c-rnd} to an arbitrary unique value}
	\STATE let \mv{c-ring} be an overlay ring with processes in a subset of $N_a \cup N_l$
	\STATE \textbf{for all} $q \in \mv{c-ring}$ \textbf{do} send ($q$, (\textsc{Phase 1a}, \mv{c-rnd}, \mv{c-ring}))
\ENDINDENT
\vspace{1.5mm}
\STATE \emph{\underline{Phase 1 (acceptor)}}
\INDENT{\textbf{upon} receiving (\textsc{Phase 1a},\mv{c-rnd},\mv{c-ring}) from coordinator}
	\INDENT{\bc{\textbf{if} $\mv{c-rnd} > \mv{rnd}$ \textbf{then}}}
		\STATE \bc{let \mv{rnd} be \mv{c-rnd}}
		\STATE let \mv{ring} be \mv{c-ring}
		\STATE \bc{send (coordinator, (\textsc{Phase 1b}, \mv{rnd}, \mv{v-rnd}, \mv{v-val}))}
	\ENDINDENT
\ENDINDENT
\vspace{1.5mm}
\STATE \emph{\underline{Phase~2 (coordinator)}}
\INDENT{\textbf{upon} receiving (\textsc{Proposal}, $v$)}
	\STATE \textbf{wait until} receiving (\textsc{Phase 1b}, \mv{rnd}, \mv{v-rnd}, \mv{v-val}) from $Q_a$ such that $\mv{rnd}=\mv{c-rnd}$
	\STATE \bc{let $k$ be the largest \mv{v-rnd} value received}
	\STATE \bc{let $V$ be the set of (\mv{v-rnd},\mv{v-val}) received with $\mv{v-rnd}\!=\!k$}
	\STATE \bc{\textbf{if} $k=0$ \textbf{then} let $\mv{c-val}$ be $v$}
	\STATE \bc{\textbf{else} let $\mv{c-val}$ be the only \mv{v-val} in $V$}
	\STATE let \mv{c-vid} be a unique identifier for \mv{c-val}
	\STATE ctr-send (\textsc{Phase 2a}, \mv{c-rnd}, \mv{c-vid})
%	\STATE msg-send (\mv{c-vid}, \mv{c-val})
	\STATE val-send (\mv{c-vid}, \mv{c-val})
\ENDINDENT
\vspace{1.5mm}
\STATE \emph{\underline{Phase~2 (acceptor)}}
\INDENT{\textbf{upon} receiving (\textsc{Phase 2a}, \mv{c-rnd}, \mv{c-vid}) \textbf{and} 
\\receiving (\mv{c-vid}, \mv{c-val})}
	\INDENT{\textbf{if} $\mv{c-rnd} \geq \mv{rnd}$ \textbf{then}}
		\STATE let \mv{v-rnd} be \mv{c-rnd}
		\STATE let \mv{v-val} be \mv{c-val}
 		\STATE let \mv{rnd} be \mv{c-rnd}
		\STATE let \mv{v-vid} be \mv{c-vid}
		\INDENT{\textbf{if} $p = \mathit{first}(ring)$ \textbf{then}}
%			\STATE send ($successor(p, ring)$, (\textsc{Phase 2b}, \mv{c-rnd}, \mv{c-vid}))
			\STATE cntr-send (\textsc{Phase 2b}, \mv{c-rnd}, \mv{c-vid})
		\ENDINDENT
	\ENDINDENT
\ENDINDENT
\vspace{1.5mm}
\STATE \emph{\underline{Phase~3 (coordinator and acceptors)}}
\INDENT{\textbf{upon} \mbox{receiving (\textsc{Phase 2b},\mv{c-rnd},\mv{c-vid})}}
	\INDENT{\textbf{if} $\mv{v-vid} = \mv{c-vid}$ \textbf{then}}
		\INDENT{\textbf{if} $p \neq last(ring)$ \textbf{then}}
%			\STATE send ($successor(p, ring)$, (\textsc{Phase 2b}, \mv{c-rnd}, \mv{c-vid}))
			\STATE cntr-send (\textsc{Phase 2b}, \mv{c-rnd}, \mv{c-vid})
		\ENDINDENT
		\INDENT{\textbf{else}}
%			\STATE ip-multicast ($Q_a \cup N_l,$ (\textsc{Decision}, \mv{c-vid}))
			\STATE msg-send (\textsc{Decision}, \mv{c-vid})
		\ENDINDENT
	\ENDINDENT
\ENDINDENT
\vspace{5mm}
\underline{Note:} \hspace{2mm}$first(ring)$: process that succeeds coordinator in $ring$\\
\hspace{10mm}$last(ring)$: the coordinator process in $ring$
%\hspace{10mm}$successor(p, ring)$: process that succeeds $p$ in $ring$
\label{alg:rpaxos}
\end{distribalgo}
\line(1,0){240}


%\end{algorithmic}

